Contiguous Patches of Translational Hydration Dynamics on the Surface of K-Ras

Proteins involved in signaling pathways represent an interesting target for experimental analysis by ODNP (Overhauser Dynamic Nuclear Polarization), which determines the translational mobility at the surface of proteins. They also represent a challenge, since the hydration dynamics at all sites remains relatively rapid, requiring sensitive measurements capable of drawing finer distinctions. Targeting the protein K-Ras, we find ODNP cross-relaxivity values that appear consistent within similar regions of 3D space, regardless of the specific residue where the spin probe used to select the location has been attached. The similar dynamics observed from nearby residues indicate a persistence/uniformity of the translational dynamics of water on the nanometer scale. This results makes sense, since it essentially means that the dynamics of water remains consistent over a lengthscale (a nanometer) over which liquid water exhibits structural persistence (i.e. its correlation length). This opens up the possibility of strategically and comprehensively mapping out the hydration layer in aqueous solution and identifying regions that contribute significantly to the free energy of binding interactions -- for example, slow water that might contribute significant entropy, or regions with strongly temperature-dependent water mobility that might contribute significant enthalpy.

==> acronyms.tex <==
%https://tex.stackexchange.com/questions/435617/glossaries-expand-acronyms-for-first-time-use-within-each-cha
\newacronym{oec}{OEC}{oxygen-evolving complex}
\newacronym{psii}{PSII}{Photosystem II}
\newacronym{lna}{LNA}{Low Noise Amplifier}
\newacronym{odnp}{ODNP}{Overhauser Dynamic Nuclear Polarization}
\newacronym{nmr}{NMR}{Nuclear Magnetic Resonance}
\newacronym{esr}{ESR}{Electron Spin Resonance}
\newacronym{deer}{DEER}{Double Electron-Electron Resonance}
\newacronym{pds}{PDS}{Pulse Dipolar Spectroscopy}
\newacronym{psd}{PSD}{Power Spectral Density}
\newacronym{eseem}{ESEEM}{Electron Spin Echo Envelope Modulation}
\newacronym{sdsl}{SDSL}{Site-Directed Spin-Labeling}
\newacronym{pre}{PRE}{Paramagnetic Relaxation Enhancement}
\newacronym{awg}{AWG}{Arbitrary Waveform Generation}
\newacronym{br}{BR}{bacteriorhodopsin}
\newacronym{pr}{PR}{proteorhodopsin}
\newacronym{md}{MD}{molecular dynamics}
\newacronym{mtsl}{MTSL}{\textit{S}-(1-oxyl-2,2,5,5-tetramethyl-2,5-dihydro-1H-pyrrol-3-yl)methyl methanesulfonothioate)}
\newacronym{ednmr}{EDNMR}{electrically detected \gls{nmr}}
\newacronym{mmm}{MMM}{the open-source Matlab tool known as Multiscale Modeling of Macromolecules}
%\newacronym{pi}{PI}{principal investigator}
\newacronym{ddm}{DDM}{n-Dodecyl-β-D-Maltopyranoside}
\newacronym{dppc}{DPPC}{dipalmitoylphosphatidylcholine}
\hyphenation{dipalmitoyl-phosphatidyl-choline}
\newacronym{dopa}{DOPA}{dioleoylphosphatidic acid}
\hyphenation{di-oleoyl-phosphatidic acid}
\newacronym{sdr}{SDR}{software-defined radio}
\newacronym{avhe}{AVHE}{Academic Virtual Hosting Environment}
\newacronym{pcet}{PCET}{proton-coupled electron transfer}
\newacronym{rnr}{RNR}{Ribonuclease reductase}
\newacronym{iq}{IQ}{quadrature}
\newacronym{sasa}{SASA}{solvent-accessible surface area}
\newacronym{mr}{MR}{Magetic Resonance}
\newacronym{dcct}{DCCT}{domain colored coherence transfer}
\newacronym{ct}{CT}{coherence transfer}
\newacronym{lp}{LP}{Linear Prediction}
\newacronym{mw}{μw}{microwave} 
\newacronym{fid}{FID}{free induction decay}
\newacronym{rm}{RM}{reverse micelle}
\newacronym{rms}{RMs}{reverse micelles}
\newacronym{snr}{SNR}{signal to noise ratio}
\newacronym{fwhm}{FWHM}{full-width-half-maximum}
\newacronym{l2g}{L2G}{Lorentzian-to-Gaussian}
\newacronym{aot}{AOT}{Aerosol-OT}
\newacronym{svd}{SVD}{Singular Value Decomposition}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{sde}{SDE}{Stokes-Debye-Einstein}
\newacronym{dls}{DLS}{Dynamic Light Scattering}
\newacronym{ctet}{\ensuremath{\text{CCl}_{4}}}{carbon tetrachloride}
\newacronym{peg}{PEG}{polyethylene glycol}
\newacronym{bsa}{BSA}{bovine serum albumin}
\newacronym{ilt}{ILT}{Inverse Laplace Transform}
\newacronym{dss}{DSS}{sodium trimethylsilylpropanesulfonate}
\newacronym{ctab}{CTAB}{cetrimonium bromide}
%g!/^%*\\.*\(paragraph\|section\)/s/[{:a-zA-Z]\@<!\([A-Z]\{2,}\)[}:a-zA-Z0-9]\@!/\\gls{\L\1}/g
% and non-expanded acronyms:
%s/\\gls{\(pi\|foa\)}/\U\1/g


==> myacronyms.tex <==
\RequirePackage[acronyms]{glossaries}
%https://tex.stackexchange.com/questions/435617/glossaries-expand-acronyms-for-first-time-use-within-each-cha
\newacronym{oec}{OEC}{oxygen-evolving complex}
\newacronym{psii}{PSII}{Photosystem II}
\newacronym{lna}{LNA}{Low Noise Amplifier}
\newacronym{odnp}{ODNP}{Overhauser Dynamic Nuclear Polarization}
\newacronym{nmr}{NMR}{Nuclear Magnetic Resonance}
\newacronym{esr}{ESR}{Electron Spin Resonance}
\newacronym{qesr}{QESR}{Quantitative Electron Spin Resonance}
\newacronym{deer}{DEER}{Double Electron-Electron Resonance}
\newacronym{pds}{PDS}{Pulse Dipolar Spectroscopy}
\newacronym{psd}{PSD}{Power Spectral Density}
\newacronym{eseem}{ESEEM}{Electron Spin Echo Envelope Modulation}
\newacronym{sdsl}{SDSL}{Site-Directed Spin-Labeling}
\newacronym{pre}{PRE}{Paramagnetic Relaxation Enhancement}
\newacronym{awg}{AWG}{Arbitrary Waveform Generation}
\newacronym{br}{BR}{bacteriorhodopsin}
\newacronym{pr}{PR}{proteorhodopsin}
\newacronym{md}{MD}{molecular dynamics}
\newacronym{mtsl}{MTSL}{\textit{S}-(1-oxyl-2,2,5,5-tetramethyl-2,5-dihydro-1H-pyrrol-3-yl)methyl methanesulfonothioate)}
\newacronym{ednmr}{EDNMR}{electrically detected \gls{nmr}}
\newacronym{mmm}{MMM}{the open-source Matlab tool known as Multiscale Modeling of Macromolecules}
%\newacronym{pi}{PI}{principal investigator}
\newacronym{ddm}{DDM}{n-Dodecyl-β-D-Maltopyranoside}
\newacronym{dppc}{DPPC}{dipalmitoylphosphatidylcholine}
\hyphenation{dipalmitoyl-phosphatidyl-choline}
\newacronym{dopa}{DOPA}{dioleoylphosphatidic acid}
\hyphenation{di-oleoyl-phosphatidic acid}
\newacronym{sdr}{SDR}{software-defined radio}
\newacronym{avhe}{AVHE}{Academic Virtual Hosting Environment}
\newacronym{pcet}{PCET}{proton-coupled electron transfer}
\newacronym{rnr}{RNR}{Ribonuclease reductase}
\newacronym{iq}{IQ}{quadrature}
\newacronym{sasa}{SASA}{solvent-accessible surface area}
\newacronym{mr}{MR}{Magnetic Resonance}
\newacronym{dcct}{DCCT}{domain colored coherence transfer}
\newacronym{ct}{CT}{coherence transfer}
\newacronym{lp}{LP}{Linear Prediction}
\newacronym{mw}{μw}{microwave} 
\newacronym{fid}{FID}{free induction decay}
\newacronym{rm}{RM}{reverse micelle}
\newacronym{rms}{RMs}{reverse micelles}
\newacronym{snr}{SNR}{signal to noise ratio}
\newacronym{fwhm}{FWHM}{full-width-half-maximum}
\newacronym{l2g}{L2G}{Lorentzian-to-Gaussian}
\newacronym{aot}{AOT}{Aerosol-OT}
\newacronym{svd}{SVD}{Singular Value Decomposition}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{sde}{SDE}{Stokes-Debye-Einstein}
\newacronym{dls}{DLS}{Dynamic Light Scattering}
\newacronym{ctet}{\ensuremath{\text{CCl}_{4}}}{carbon tetrachloride}
\newacronym{peg}{PEG}{polyethylene glycol}
\newacronym{bsa}{BSA}{bovine serum albumin}
\newacronym{ilt}{ILT}{Inverse Laplace Transform}
\newacronym{dss}{DSS}{sodium trimethylsilylpropanesulfonate}
\newacronym{ctab}{CTAB}{cetrimonium bromide}
%g!/^%*\\.*\(paragraph\|section\)/s/[{:a-zA-Z]\@<!\([A-Z]\{2,}\)[}:a-zA-Z0-9]\@!/\\gls{\L\1}/g
% and non-expanded acronyms:
%s/\\gls{\(pi\|foa\)}/\U\1/g

